Dragonfly: a modular deep reinforcement learning library

Dragonfly is a deep reinforcement learning library focused on modularity, in order to ease experimentation and developments. It relies on a json serialization that allows to swap building blocks and perform parameter sweep, while minimizing code maintenance. Some of its features are specifically designed for CPU-intensive environments, such as numerical simulations. Its performance on standard agents using common benchmarks compares favorably with the literature.

==> fig/mixing/mixing_example.tex <==
%%%%%%%%%%%%
%%%%%%%%%%%%
\begin{figure}
\centering
%%%%%%%%%%%%
\pgfdeclarelayer{background}
\pgfsetlayers{background,main}
%%%%%%%%%%%%
%%%%%%%%%%%%

\begin{subfigure}[t]{.22\textwidth}
	\centering
	\fbox{\includegraphics[width=\textwidth]{fig/mixing/mixing_example_t0.png}}
    	\caption{$t=0$}
	\label{fig:mixing_example_0}
\end{subfigure} \quad
\begin{subfigure}[t]{.22\textwidth}
	\centering
	\fbox{\includegraphics[width=\textwidth]{fig/mixing/mixing_example_t10.png}}
    	\caption{$t=10$}
	\label{fig:mixing_example_10}
\end{subfigure} \quad
\begin{subfigure}[t]{.22\textwidth}
	\centering
	\fbox{\includegraphics[width=\textwidth]{fig/mixing/mixing_example_t30.png}}
    	\caption{$t=30$}
	\label{fig:mixing_example_30}
\end{subfigure} \quad
\begin{subfigure}[t]{.22\textwidth}
	\centering
	\fbox{\includegraphics[width=\textwidth]{fig/mixing/mixing_example_t60.png}}
    	\caption{$t=60$}
	\label{fig:mixing_example_60}
\end{subfigure}

%%%%%%%%%%%%
\caption{\textbf{Evolution of the concentration in time} with constant boundary conditions.}
\label{fig:mixing_example}
\end{figure} 
%%%%%%%%%%%%
%%%%%%%%%%%%

==> fig/mixing/mixing_obs.tex <==
%%%%%%%%%%%%
%%%%%%%%%%%%
\begin{figure}
\centering
%%%%%%%%%%%%
\pgfdeclarelayer{background}
\pgfsetlayers{background,main}
%%%%%%%%%%%%
%%%%%%%%%%%%

\begin{subfigure}[t]{\textwidth}
	%\centering
	\includegraphics[height=.5cm,width=\textwidth]{fig/mixing/obs_original.png}
\end{subfigure}

%%%%%%%%%%%%

\begin{subfigure}[t]{\textwidth}
	%\centering
	\includegraphics[height=.5cm,width=.05\textwidth]{fig/mixing/obs_pca.png}
\end{subfigure}

%\begin{subfigure}[t]{\textwidth}
%	%\centering
%	\includegraphics[width=.4\textwidth]{fig/shkadov/obs_ae.png}
%\end{subfigure}

%%%%%%%%%%%%
\caption{\textbf{Observations standard deviation averaged over one episode} with \textsc{ppo} (top), \textsc{ppo-pca} (middle), and \textsc{ppo-ae} (bottom). Values are scaled between $0$ (deep blue) to $1$ (red).}
\label{fig:mixing_obs}
\end{figure} 
%%%%%%%%%%%%
%%%%%%%%%%%%

==> fig/mixing/mixing_pca.tex <==
%%%%%%%%%%%%
%%%%%%%%%%%%
\begin{figure}
\centering
%%%%%%%%%%%%
\begin{subfigure}[t]{.35\textwidth}
\centering
\begin{tikzpicture}[	trim axis left, trim axis right, font=\scriptsize,
				upper/.style={	name path=upper, smooth, draw=none},
				lower/.style={	name path=lower, smooth, draw=none},]
	\begin{axis}[	xmin=0, xmax=150000, scale=0.7,
				ymin=-20, ymax=-5,
				scaled x ticks=false, scaled y ticks=false,
				xtick={0,50000,100000,150000},
				xticklabels={$0$,$50k$,$100k$,$150k$},
				legend cell align=left, legend pos=south east,
				legend style={nodes={scale=0.8, transform shape}},
				every tick label/.append style={font=\scriptsize},
				grid=major, xlabel=transitions, ylabel=score]
				
		\legend{\textsc{ppo}(10000), \textsc{ppo-cnn}(10000), \textsc{ppo-cae}(500), \textsc{ppo-pca}(500)}
		
		\addplot[upper, forget plot] 				table[x index=0,y index=7] {fig/mixing/ppo_100x100.dat};
		\addplot[lower, forget plot] 				table[x index=0,y index=6] {fig/mixing/ppo_100x100.dat}; 
		\addplot[fill=gray3, opacity=0.5, forget plot] 	fill between[of=upper and lower];
		\addplot[draw=gray1, thick, smooth] 			table[x index=0,y index=5] {fig/mixing/ppo_100x100.dat};
		
  	      	\addplot [upper, forget plot] 				table[x index=0,y index=7] {fig/mixing/ppo_100x100_cnn.dat};
		\addplot [lower, forget plot] 				table[x index=0,y index=6] {fig/mixing/ppo_100x100_cnn.dat};
		\addplot [fill=purple3, opacity=0.5, forget plot] 	fill between[of=upper and lower];
		\addplot[draw=purple1, thick, smooth] 		table[x index=0,y index=5] {fig/mixing/ppo_100x100_cnn.dat};
		
  	      	\addplot [upper, forget plot] 				table[x index=0,y index=7] {fig/mixing/ppo_100x100_cae.dat};
		\addplot [lower, forget plot] 				table[x index=0,y index=6] {fig/mixing/ppo_100x100_cae.dat};
		\addplot [fill=blue3, opacity=0.5, forget plot] 	fill between[of=upper and lower];
		\addplot[draw=blue1, thick, smooth] 			table[x index=0,y index=5] {fig/mixing/ppo_100x100_cae.dat};
		
  	      	\addplot [upper, forget plot] 				table[x index=0,y index=7] {fig/mixing/ppo_100x100_pca.dat};
		\addplot [lower, forget plot] 				table[x index=0,y index=6] {fig/mixing/ppo_100x100_pca.dat};
		\addplot [fill=red3, opacity=0.5, forget plot] 	fill between[of=upper and lower];
		\addplot[draw=red1, thick, smooth] 			table[x index=0,y index=5] {fig/mixing/ppo_100x100_pca.dat};
		
	\end{axis}
\end{tikzpicture}
\caption{Score curves}
\label{fig:mixing_ppo_pca_score}
\end{subfigure} \qquad \qquad
%%%%%%%%%%%%
\begin{subfigure}[t]{.35\textwidth}
\centering
\begin{tikzpicture}[	trim axis left, trim axis right, font=\scriptsize]
	\begin{semilogyaxis}[	xmin=0, xmax=16000, scale=0.7,
						%ymin=0.0001, ymax=2,
						%xtick={10,100,1000},
						%xticklabels={10,100,1000},
						legend style={nodes={scale=0.8, transform shape}},
						scaled x ticks=false, scaled y ticks=false,
						every tick label/.append style={font=\scriptsize},
						grid=major, xlabel=epochs, ylabel=loss]
						
		\legend{\textsc{ppo-cae}(500)}
		
		\addplot[draw=teal1, thick, smooth] table[x index=0,y index=1] {fig/mixing/cae_loss.dat };
%		\addplot[draw=blue1, thick, smooth] table[x index=0,y index=1] {fig/shkadov/ae_loss_dim_100.dat};
%		\addplot[draw=red1, thick, smooth] table[x index=0,y index=1] {fig/shkadov/ae_loss_dim_500.dat};
		
	\end{semilogyaxis}
\end{tikzpicture}
\caption{Loss curves}
\label{fig:mixing_ppo_cae_loss_curves}
\end{subfigure}
%%%%%%%%%%%%

\medskip
\medskip

%%%%%%%%%%%%
\begin{subfigure}[t]{.35\textwidth}
\centering
\begin{tikzpicture}[	trim axis left, trim axis right, font=\scriptsize]
	\begin{axis}[	view={0}{90}, scale=0.7, colormap/RdBu,
				scaled x ticks=false, scaled y ticks=false,
				every tick label/.append style={font=\scriptsize},
				grid=major, xlabel=latent dimension 1, ylabel=latent dimension 2]
		
		\addplot3[only marks, scatter, mark=*,mark size=1pt] table[x index=1, y index=2, z index=0] {fig/mixing/pca_2d};
		
	\end{axis}
\end{tikzpicture}
\caption{Representation of an episode in a \textsc{2d} \textsc{pca} latent space}
\label{fig:shkadov_ppo_pca_episode}
\end{subfigure}
%%%%%%%%%%%%
\caption{\textbf{Comparing} \textsc{ppo} \textbf{with} \textsc{ppo-pca} \textbf{on the mixing environment } with increasing latent space dimensions. On the left, blabla, on the right, blabla.} 
\label{fig:shkadov_ppo_pca}
\end{figure} 
%%%%%%%%%%%%
%%%%%%%%%%%%

==> fig/parallel/parallel.tex <==
%%%%%%%%%%%%
\begin{figure}[h!]
\centering
\def\nsteps{200000}
%%%%%%%%%%%%
\begin{subfigure}[t]{.55\textwidth}
\centering
  \begin{tikzpicture}[	trim axis left, trim axis right, font=\scriptsize,
          upper/.style={	name path=upper, smooth, draw=none},
          lower/.style={	name path=lower, smooth, draw=none},
          limit/.style={	gray3, thick, dash pattern=on 2pt}]
    \begin{axis}[	xmin=0, xmax=90, ymin=-4, ymax=0, scale=0.8,
          width=\textwidth, height=5cm, scale only axis=true,
          every tick label/.append style={font=\scriptsize},
          legend cell align=left, legend pos=south east,
          grid=major, xlabel=training minutes, ylabel=score]

      \legend{1 env, 2 envs, 4 envs, 8 envs, 16 envs, 32 envs, 64 envs}

      % 1 env
      \def\tun{5380}
      \addplot [upper, forget plot]         table[x expr=\thisrowno{0}/\nsteps*\tun/60,y index=7] {fig/shkadov_1_env_no_bs.dat};
      \addplot [lower, forget plot]         table[x expr=\thisrowno{0}/\nsteps*\tun/60,y index=6] {fig/shkadov_1_env_no_bs.dat};
      \addplot [fill=teal3, opacity=0.5, forget plot]   fill between[of=upper and lower];
      \addplot[draw=teal1, thick, smooth]       table[x expr=\thisrowno{0}/\nsteps*\tun/60,y index=5] {fig/shkadov_1_env_no_bs.dat};
      \addplot[limit, forget plot]					coordinates {(\tun/60,-4) (\tun/60,0)};

      % 2 env
      \def\ttwo{2834}
      \addplot [upper, forget plot]         table[x expr=\thisrowno{0}/\nsteps*\ttwo/60,y index=7] {fig/shkadov_2_envs_no_bs.dat};
      \addplot [lower, forget plot]         table[x expr=\thisrowno{0}/\nsteps*\ttwo/60,y index=6] {fig/shkadov_2_envs_no_bs.dat};
      \addplot [fill=red3, opacity=0.5, forget plot]  fill between[of=upper and lower];
      \addplot[draw=red1, thick, smooth]      table[x expr=\thisrowno{0}/\nsteps*\ttwo/60,y index=5] {fig/shkadov_2_envs_no_bs.dat};
      \addplot[limit, forget plot]					coordinates {(\ttwo/60,-4) (\ttwo/60,0)};

      % 4 env
      \def\tfour{1470}
      \addplot [upper, forget plot]         table[x expr=\thisrowno{0}/\nsteps*\tfour/60,y index=7] {fig/shkadov_4_envs_no_bs.dat};
      \addplot [lower, forget plot]         table[x expr=\thisrowno{0}/\nsteps*\tfour/60,y index=6] {fig/shkadov_4_envs_no_bs.dat};
      \addplot [fill=gray3, opacity=0.5, forget plot]   fill between[of=upper and lower];
      \addplot[draw=gray1, thick, smooth]       table[x expr=\thisrowno{0}/\nsteps*\tfour/60,y index=5] {fig/shkadov_4_envs_no_bs.dat};
      \addplot[limit, forget plot]					coordinates {(\tfour/60,-4) (\tfour/60,0)};

      % 8 envs
      \def\thuit{775}
      \addplot [upper, forget plot]         table[x expr=\thisrowno{0}/\nsteps*\thuit/60,y index=7] {fig/shkadov_8_envs_no_bs.dat};
      \addplot [lower, forget plot]         table[x expr=\thisrowno{0}/\nsteps*\thuit/60,y index=6] {fig/shkadov_8_envs_no_bs.dat};
      \addplot [fill=blue3, opacity=0.5, forget plot]   fill between[of=upper and lower];
      \addplot[draw=blue1, thick, smooth]       table[x expr=\thisrowno{0}/\nsteps*\thuit/60,y index=5] {fig/shkadov_8_envs_no_bs.dat};
      \addplot[limit, forget plot]					coordinates {(\thuit/60,-4) (\thuit/60,0)};

      % 16 envs
      \def\tseize{441}
      \addplot [upper, forget plot]           table[x expr=\thisrowno{0}/\nsteps*\tseize/60,y index=7] {fig/shkadov_16_envs_no_bs.dat};
      \addplot [lower, forget plot]           table[x expr=\thisrowno{0}/\nsteps*\tseize/60,y index=6] {fig/shkadov_16_envs_no_bs.dat};
      \addplot [fill=bluegray3, opacity=0.5, forget plot]   fill between[of=upper and lower];
      \addplot[draw=bluegray1, thick, smooth]       table[x expr=\thisrowno{0}/\nsteps*\tseize/60,y index=5] {fig/shkadov_16_envs_no_bs.dat};
      \addplot[limit, forget plot]						coordinates {(\tseize/60,-4) (\tseize/60,0)};

      % 32 envs
      \def\ttdeux{304}
      \addplot [upper, forget plot]         table[x expr=\thisrowno{0}/\nsteps*\ttdeux/60,y index=7] {fig/shkadov_32_envs_no_bs.dat};
      \addplot [lower, forget plot]         table[x expr=\thisrowno{0}/\nsteps*\ttdeux/60,y index=6] {fig/shkadov_32_envs_no_bs.dat};
      \addplot [fill=orange3, opacity=0.5, forget plot]   fill between[of=upper and lower];
      \addplot[draw=orange1, thick, smooth]     table[x expr=\thisrowno{0}/\nsteps*\ttdeux/60,y index=5] {fig/shkadov_32_envs_no_bs.dat};
      \addplot[limit, forget plot]					coordinates {(\ttdeux/60,-4) (\ttdeux/60,0)};

      % 64 envs
      \def\tsquatre{293}
      \addplot [upper, forget plot]         table[x expr=\thisrowno{0}/\nsteps*\tsquatre/60,y index=7] {fig/shkadov_64_envs_no_bs.dat};
      \addplot [lower, forget plot]         table[x expr=\thisrowno{0}/\nsteps*\tsquatre/60,y index=6] {fig/shkadov_64_envs_no_bs.dat};
      \addplot [fill=purple3, opacity=0.5, forget plot]   fill between[of=upper and lower];
      \addplot[draw=purple1, thick, smooth]     table[x expr=\thisrowno{0}/\nsteps*\tsquatre/60,y index=5] {fig/shkadov_64_envs_no_bs.dat};
      \addplot[limit, forget plot]					coordinates {(\tsquatre/60,-4) (\tsquatre/60,0)};

    \end{axis}
  \end{tikzpicture}
  \caption{Score against walltime, no bootstrapping}
\end{subfigure} \quad
%%%%%%%%%%%%
\begin{subfigure}[t]{.35\textwidth}
\centering
  \begin{tikzpicture}[	trim axis left, trim axis right, font=\scriptsize,
          upper/.style={	name path=upper, smooth, draw=none},
          lower/.style={	name path=lower, smooth, draw=none},]
    \begin{axis}[	xmin=0, xmax=200000, ymin=-4, ymax=0, scale=0.8,
          xtick={0,50000,100000,150000,200000},
          xticklabels={$0$,$50k$,$100k$,$150k$,$200k$},
          scaled x ticks=false,
          width=\textwidth, height=5cm, scale only axis=true,
          every tick label/.append style={font=\scriptsize},
          legend cell align=left, legend pos=south east,
          grid=major, xlabel=transitions, ylabel={}]

      % 1 env
      \addplot [upper, forget plot]         table[x index=0,y index=7] {fig/shkadov_1_env_no_bs.dat};
      \addplot [lower, forget plot]         table[x index=0,y index=6] {fig/shkadov_1_env_no_bs.dat};
      \addplot [fill=teal3, opacity=0.5, forget plot]   fill between[of=upper and lower];
      \addplot[draw=teal1, thick, smooth]       table[x index=0,y index=5] {fig/shkadov_1_env_no_bs.dat};

      % 2 env
      \addplot [upper, forget plot]         table[x index=0,y index=7] {fig/shkadov_2_envs_no_bs.dat};
      \addplot [lower, forget plot]         table[x index=0,y index=6] {fig/shkadov_2_envs_no_bs.dat};
      \addplot [fill=red3, opacity=0.5, forget plot]  fill between[of=upper and lower];
      \addplot[draw=red1, thick, smooth]      table[x index=0,y index=5] {fig/shkadov_2_envs_no_bs.dat};

      % 4 env
      \addplot [upper, forget plot]         table[x index=0,y index=7] {fig/shkadov_4_envs_no_bs.dat};
      \addplot [lower, forget plot]         table[x index=0,y index=6] {fig/shkadov_4_envs_no_bs.dat};
      \addplot [fill=gray3, opacity=0.5, forget plot]   fill between[of=upper and lower];
      \addplot[draw=gray1, thick, smooth]       table[x index=0,y index=5] {fig/shkadov_4_envs_no_bs.dat};

      % 8 envs
      \addplot [upper, forget plot]         table[x index=0,y index=7] {fig/shkadov_8_envs_no_bs.dat};
      \addplot [lower, forget plot]         table[x index=0,y index=6] {fig/shkadov_8_envs_no_bs.dat};
      \addplot [fill=blue3, opacity=0.5, forget plot]   fill between[of=upper and lower];
      \addplot[draw=blue1, thick, smooth]       table[x index=0,y index=5] {fig/shkadov_8_envs_no_bs.dat};

      % 16 envs
      \addplot [upper, forget plot]           table[x index=0,y index=7] {fig/shkadov_16_envs_no_bs.dat};
      \addplot [lower, forget plot]           table[x index=0,y index=6] {fig/shkadov_16_envs_no_bs.dat};
      \addplot [fill=bluegray3, opacity=0.5, forget plot]   fill between[of=upper and lower];
      \addplot[draw=bluegray1, thick, smooth]       table[x index=0,y index=5] {fig/shkadov_16_envs_no_bs.dat};

      % 32 envs
      \addplot [upper, forget plot]           table[x index=0,y index=7] {fig/shkadov_32_envs_no_bs.dat};
      \addplot [lower, forget plot]           table[x index=0,y index=6] {fig/shkadov_32_envs_no_bs.dat};
      \addplot [fill=orange3, opacity=0.5, forget plot]     fill between[of=upper and lower];
      \addplot[draw=orange1, thick, smooth]       table[x index=0,y index=5] {fig/shkadov_32_envs_no_bs.dat};

      % 64 envs
      \addplot [upper, forget plot]           table[x index=0,y index=7] {fig/shkadov_64_envs_no_bs.dat};
      \addplot [lower, forget plot]           table[x index=0,y index=6] {fig/shkadov_64_envs_no_bs.dat};
      \addplot [fill=purple3, opacity=0.5, forget plot]     fill between[of=upper and lower];
      \addplot[draw=purple1, thick, smooth]       table[x index=0,y index=5] {fig/shkadov_64_envs_no_bs.dat};

    \end{axis}
  \end{tikzpicture}
  \caption{Score against transitions, no bootstrapping}
\end{subfigure}
%%%%%%%%%%%%

\medskip

%%%%%%%%%%%%
\begin{subfigure}[t]{.55\textwidth}
\centering
  \begin{tikzpicture}[	trim axis left, trim axis right, font=\scriptsize,
          upper/.style={	name path=upper, smooth, draw=none},
          lower/.style={	name path=lower, smooth, draw=none},
          limit/.style={	gray3, thick, dash pattern=on 2pt}]
    \begin{axis}[	xmin=0, xmax=90, ymin=-4, ymax=0, scale=0.8,
          width=\textwidth, height=5cm, scale only axis=true,
          every tick label/.append style={font=\scriptsize},
          legend cell align=left, legend pos=south east,
          grid=major, xlabel=training minutes, ylabel=score]

      \legend{1 env, 2 envs, 4 envs, 8 envs, 16 envs, 32 envs, 64 envs}

      % 1 env
      \def\tun{5254}
      \addplot [upper, forget plot]         table[x expr=\thisrowno{0}/\nsteps*\tun/60,y index=7] {fig/shkadov_1_env_bs.dat};
      \addplot [lower, forget plot]         table[x expr=\thisrowno{0}/\nsteps*\tun/60,y index=6] {fig/shkadov_1_env_bs.dat};
      \addplot [fill=teal3, opacity=0.5, forget plot]   fill between[of=upper and lower];
      \addplot[draw=teal1, thick, smooth]       table[x expr=\thisrowno{0}/\nsteps*\tun/60,y index=5] {fig/shkadov_1_env_bs.dat};
      \addplot[limit, forget plot]					coordinates {(\tun/60,-4) (\tun/60,0)};

      % 2 env
      \def\ttwo{2642}
      \addplot [upper, forget plot]         table[x expr=\thisrowno{0}/\nsteps*\ttwo/60,y index=7] {fig/shkadov_2_envs_bs.dat};
      \addplot [lower, forget plot]         table[x expr=\thisrowno{0}/\nsteps*\ttwo/60,y index=6] {fig/shkadov_2_envs_bs.dat};
      \addplot [fill=red3, opacity=0.5, forget plot]  fill between[of=upper and lower];
      \addplot[draw=red1, thick, smooth]      table[x expr=\thisrowno{0}/\nsteps*\ttwo/60,y index=5] {fig/shkadov_2_envs_bs.dat};
      \addplot[limit, forget plot]					coordinates {(\ttwo/60,-4) (\ttwo/60,0)};

      % 4 env
      \def\tfour{1341}
      \addplot [upper, forget plot]         table[x expr=\thisrowno{0}/\nsteps*\tfour/60,y index=7] {fig/shkadov_4_envs_bs.dat};
      \addplot [lower, forget plot]         table[x expr=\thisrowno{0}/\nsteps*\tfour/60,y index=6] {fig/shkadov_4_envs_bs.dat};
      \addplot [fill=gray3, opacity=0.5, forget plot]   fill between[of=upper and lower];
      \addplot[draw=gray1, thick, smooth]       table[x expr=\thisrowno{0}/\nsteps*\tfour/60,y index=5] {fig/shkadov_4_envs_bs.dat};
      \addplot[limit, forget plot]					coordinates {(\tfour/60,-4) (\tfour/60,0)};

      % 8 envs
      \def\thuit{695}
      \addplot [upper, forget plot]         table[x expr=\thisrowno{0}/\nsteps*\thuit/60,y index=7] {fig/shkadov_8_envs_bs.dat};
      \addplot [lower, forget plot]         table[x expr=\thisrowno{0}/\nsteps*\thuit/60,y index=6] {fig/shkadov_8_envs_bs.dat};
      \addplot [fill=blue3, opacity=0.5, forget plot]   fill between[of=upper and lower];
      \addplot[draw=blue1, thick, smooth]       table[x expr=\thisrowno{0}/\nsteps*\thuit/60,y index=5] {fig/shkadov_8_envs_bs.dat};
      \addplot[limit, forget plot]					coordinates {(\thuit/60,-4) (\thuit/60,0)};

      % 16 envs
      \def\tseize{370}
      \addplot [upper, forget plot]           table[x expr=\thisrowno{0}/\nsteps*\tseize/60,y index=7] {fig/shkadov_16_envs_bs.dat};
      \addplot [lower, forget plot]           table[x expr=\thisrowno{0}/\nsteps*\tseize/60,y index=6] {fig/shkadov_16_envs_bs.dat};
      \addplot [fill=bluegray3, opacity=0.5, forget plot]   fill between[of=upper and lower];
      \addplot[draw=bluegray1, thick, smooth]       table[x expr=\thisrowno{0}/\nsteps*\tseize/60,y index=5] {fig/shkadov_16_envs_bs.dat};
      \addplot[limit, forget plot]						coordinates {(\tseize/60,-4) (\tseize/60,0)};

      % 32 envs
      \def\ttdeux{215}
      \addplot [upper, forget plot]         table[x expr=\thisrowno{0}/\nsteps*\ttdeux/60,y index=7] {fig/shkadov_32_envs_bs.dat};
      \addplot [lower, forget plot]         table[x expr=\thisrowno{0}/\nsteps*\ttdeux/60,y index=6] {fig/shkadov_32_envs_bs.dat};
      \addplot [fill=orange3, opacity=0.5, forget plot]   fill between[of=upper and lower];
      \addplot[draw=orange1, thick, smooth]     table[x expr=\thisrowno{0}/\nsteps*\ttdeux/60,y index=5] {fig/shkadov_32_envs_bs.dat};
      \addplot[limit, forget plot]					coordinates {(\ttdeux/60,-4) (\ttdeux/60,0)};

      % 64 envs
      \def\tsquatre{124}
      \addplot [upper, forget plot]         table[x expr=\thisrowno{0}/\nsteps*\tsquatre/60,y index=7] {fig/shkadov_64_envs_bs.dat};
      \addplot [lower, forget plot]         table[x expr=\thisrowno{0}/\nsteps*\tsquatre/60,y index=6] {fig/shkadov_64_envs_bs.dat};
      \addplot [fill=purple3, opacity=0.5, forget plot]   fill between[of=upper and lower];
      \addplot[draw=purple1, thick, smooth]     table[x expr=\thisrowno{0}/\nsteps*\tsquatre/60,y index=5] {fig/shkadov_64_envs_bs.dat};
      \addplot[limit, forget plot]					coordinates {(\tsquatre/60,-4) (\tsquatre/60,0)};

    \end{axis}
  \end{tikzpicture}
  \caption{Score against walltime, parallel bootstrapping}
\end{subfigure} \quad
%%%%%%%%%%%%
\begin{subfigure}[t]{.35\textwidth}
\centering
  \begin{tikzpicture}[	trim axis left, trim axis right, font=\scriptsize,
          upper/.style={	name path=upper, smooth, draw=none},
          lower/.style={	name path=lower, smooth, draw=none},]
    \begin{axis}[	xmin=0, xmax=200000, ymin=-4, ymax=0, scale=0.8,
          xtick={0,50000,100000,150000,200000},
          xticklabels={$0$,$50k$,$100k$,$150k$,$200k$},
          scaled x ticks=false,
          width=\textwidth, height=5cm, scale only axis=true,
          every tick label/.append style={font=\scriptsize},
          legend cell align=left, legend pos=south east,
          grid=major, xlabel=transitions, ylabel={}]

      % 1 env
      \addplot [upper, forget plot]         table[x index=0,y index=7] {fig/shkadov_1_env_bs.dat};
      \addplot [lower, forget plot]         table[x index=0,y index=6] {fig/shkadov_1_env_bs.dat};
      \addplot [fill=teal3, opacity=0.5, forget plot]   fill between[of=upper and lower];
      \addplot[draw=teal1, thick, smooth]   table[x index=0,y index=5] {fig/shkadov_1_env_bs.dat};

      % 2 env
      \addplot [upper, forget plot]         table[x index=0,y index=7] {fig/shkadov_2_envs_bs.dat};
      \addplot [lower, forget plot]         table[x index=0,y index=6] {fig/shkadov_2_envs_bs.dat};
      \addplot [fill=red3, opacity=0.5, forget plot]  fill between[of=upper and lower];
      \addplot[draw=red1, thick, smooth]    table[x index=0,y index=5] {fig/shkadov_2_envs_bs.dat};

      % 4 env
      \addplot [upper, forget plot]         table[x index=0,y index=7] {fig/shkadov_4_envs_bs.dat};
      \addplot [lower, forget plot]         table[x index=0,y index=6] {fig/shkadov_4_envs_bs.dat};
      \addplot [fill=gray3, opacity=0.5, forget plot]   fill between[of=upper and lower];
      \addplot[draw=gray1, thick, smooth]   table[x index=0,y index=5] {fig/shkadov_4_envs_bs.dat};

      % 8 envs
      \addplot [upper, forget plot]         table[x index=0,y index=7] {fig/shkadov_8_envs_bs.dat};
      \addplot [lower, forget plot]         table[x index=0,y index=6] {fig/shkadov_8_envs_bs.dat};
      \addplot [fill=blue3, opacity=0.5, forget plot]   fill between[of=upper and lower];
      \addplot[draw=blue1, thick, smooth]   table[x index=0,y index=5] {fig/shkadov_8_envs_bs.dat};

      % 16 envs
      \addplot [upper, forget plot]           table[x index=0,y index=7] {fig/shkadov_16_envs_bs.dat};
      \addplot [lower, forget plot]           table[x index=0,y index=6] {fig/shkadov_16_envs_bs.dat};
      \addplot [fill=bluegray3, opacity=0.5, forget plot]   fill between[of=upper and lower];
      \addplot[draw=bluegray1, thick, smooth] table[x index=0,y index=5] {fig/shkadov_16_envs_bs.dat};

      % 32 envs
      \addplot [upper, forget plot]           table[x index=0,y index=7] {fig/shkadov_32_envs_bs.dat};
      \addplot [lower, forget plot]           table[x index=0,y index=6] {fig/shkadov_32_envs_bs.dat};
      \addplot [fill=orange3, opacity=0.5, forget plot]     fill between[of=upper and lower];
      \addplot[draw=orange1, thick, smooth]   table[x index=0,y index=5] {fig/shkadov_32_envs_bs.dat};

      % 64 envs
      \addplot [upper, forget plot]           table[x index=0,y index=7] {fig/shkadov_64_envs_bs.dat};
      \addplot [lower, forget plot]           table[x index=0,y index=6] {fig/shkadov_64_envs_bs.dat};
      \addplot [fill=purple3, opacity=0.5, forget plot]     fill between[of=upper and lower];
      \addplot[draw=purple1, thick, smooth]   table[x index=0,y index=5] {fig/shkadov_64_envs_bs.dat};

    \end{axis}
  \end{tikzpicture}
  \caption{Score against transitions, parallel bootstrapping}
\end{subfigure}
%%%%%%%%%%%%
\caption{\textbf{Score curves obtained for different number of parallel environments} on the \codeinline{shkadov-v0} environment from the \textsc{beacon} benchmark\cite{beacon}. The agent is updated with $4$ full trajectories. (Top) With no bootstrapping, the learning rate and the final performance decrease significantly beyond $4$ parallel environemnts (Bottom) With bootstrapping, performance is maintained exactly up to $16$ parallel environments, and with a very slight performance decrease up to $32$ parallel environments.}
\label{fig:parallel}
\end{figure}


==> results.tex <==
\section{Results}
\subsection{Shkadov}

We consider the training of the PPO agent with and without SRL module on the \verb+shkadov-v0+ environment. 



\input{fig/shkadov/shkadov_ae}

\input{fig/shkadov/shkadov_fields}

\input{fig/shkadov/shkadov_obs}

\subsubsection{Mixing}



\input{fig/mixing/mixing_obs}

